A Framework for Active Haptic Guidance Using Robotic Haptic Proxies

Haptic feedback is an important component of creating an immersive mixed reality experience. Traditionally, haptic forces are rendered in response to the user's interactions with the virtual environment. In this work, we explore the idea of rendering haptic forces in a proactive manner, with the explicit intention to influence the user's behavior through compelling haptic forces. To this end, we present a framework for active haptic guidance in mixed reality, using one or more robotic haptic proxies to influence user behavior and deliver a safer and more immersive virtual experience. We provide details on common challenges that need to be overcome when implementing active haptic guidance, and discuss example applications that show how active haptic guidance can be used to influence the user's behavior. Finally, we apply active haptic guidance to a virtual reality navigation problem, and conduct a user study that demonstrates how active haptic guidance creates a safer and more immersive experience for users.

==> methods_old.tex <==

\section{PROBLEM STATEMENT}
% apply haptic force to guide the user
% make this haptic force align with objects in the virtual world
% effectiveness of haptic guidance: depends on the strength/rendering of the haptic force AND on the associated virtual object of interest. some are better at capturing the user's attention than others.
In this section, we provide a formalization of the active haptic guidance problem for users in virtual reality (VR).
The active haptic guidance problem involves two main goals for our robots.
First, the robots aim to provide haptic feedback to the user in order to guide them to a specific goal configuration in the physical and/or virtual environment.
Second, to deliver an immersive experience, the haptic feedback must align with objects in the virtual environment that the user interacts with.

Let $O = \{o_1, o_2, ..., o_i\}$ be a set of polygonal objects with vertices in $\mathbb{R}^3$.
Let $U = \{u_1, u_2, ..., u_j\}$ be the set of users in an environment.
Here, $u = \{p, \theta\}$ represents a user's state in the environment, where $p \in \mathbb{R}^3$ represents their position and $\theta \in [0, 2\pi)$ represents their orientation in the environment.
Let $R = \{ r_1, r_2, ..., r_k \}$ be the set of robots in an environment.
Let $A = \{U \cup R\}$ be set of all agents, defined as the union of the users and robots in an environment.
Each of these sets $O, U, R, \text{and } A$ may be empty.
We define an environment $E$ as a set of obstacles and agents; that is, $E = \{O, A\}$.
To differentiate between the PE and VE, we denote the PE as $E_P = \{O_P, A_P \}$ and the VE as $E_V = \{O_V, A_V \}$.
For each user in virtual reality, they will have a representation in both the PE and VE, so $|U_P| = |U_V| = n$, where $n$ is the number of users in virtual reality.

\subsection{Haptic Guidance to a Goal Configuration}
In virtual reality, we often want to reposition the user in the physical and virtual environments to ensure their safety (e.g. reposition the user so that they do not walk into nearby physical objects that they cannot see) and to improve their virtual experience (e.g. the user may need to be directed to a specific area in the virtual environment to advance their progression in a VR game).
Typical methods for repositioning users to ensure their safety involve pausing the virtual experience and displaying warnings in the head-mounted display that instruct users to adjust their positioning.
While this is effective, it is unnatural and tends to reduce the users' feelings of presence within the virtual experience.
Similarly, to direct users to specific locations in the virtual world, developers often make use of narrative story telling elements to grab and guide the users' attention, but they are usually limited to visual stimuli and cannot take advantage of haptic stimuli that can enhance the users' sense of presence.
In this work, we utilize mobile robots to provide haptic feedback to VR users to help ensure their safety in the physical space and improve their immersion in the virtual experience.

Given a user's current configuration $u^c$, there is a goal configuration $u^g$ that we want the user to adopt.
To achieve this, we need to apply haptic force $F$ to the user's haptic output device.
The user responds to this force by repositioning themself, hopefully in a direction that moves them towards $u^g$.
In this work, the haptic force $F$ is rendered through a leash tether that the user holds.
When the robot attached to the other end of the leash moves away from the user, it creates a pulling force on the leash which encourages the user to follow the robot, guiding them towards the desired position in the physical space.

\subsection{Relative Co-location Between Virtual Objects and Robot Agents}
In order to increase the plausibility of the haptic forces a user experiences, we need to align the forces with objects in the virtual environment such that the user perceives these objects to be the source of the haptic forces they feel. 
For a given user in the VE, there is a set of ``obstacles of interest'' that the user is likely to interact with.
We denote this set of obstacles as $\mathcal{O}$; note that $\mathcal{O} \subset O_V$.
The active haptic guidance problem can then be stated as updating the configurations of physical robots $R$ such that their configuration matches with the configurations of nearby objects of interest that a user is likely to interact with.
That is, we wish to reposition and reorient the robots in the PE to match the positions of objects of interest \textit{relative to the user's configuration}.
We can cast this as a motion planning problem, where the goal is to find paths for the robots in the PE that reconfigures them to be as close as possible to the configurations of the objects of interest in the VE.

% emphasize that this is a user-centric problem. all robot manipulation is done in service of the user experience, in order to provide the appropriate haptic feedback. we use this haptic feedback to guide the user to a target configuration in the physica/virtual environment.

% a bunch of math that defines the problem.
% one user, virtual environment, physical environment, virtual objects for which we want haptic feedback, and n robots that provide said haptic feedback.
% not every element/object/agent in the virtual environment will have a physical counterpart.
% need to compute the correct position of each robot relative to the user in the physical environment in real time.
% this position is determined by constraints (location of the robot's virtual agent relative to the virtual user, other constraints on the relationship between the user and the virtual agent (e.g. tether like robot dog)).



